Are Machine Programming Systems using Right Source-Code Measures to Select Code Repositories?

Machine programming (MP) is an emerging field at the intersection of deterministic and probabilistic computing, and it aims to assist software and hardware engineers, among other applications. Along with powerful compute resources, MP systems often rely on vast amount of open-source code to learn interesting properties about code and programming and solve problems in the areas of debugging, code recommendation, auto-completion, etc. Unfortunately, several of the existing MP systems either do not consider quality of code repositories or use atypical quality measures than those typically used in software engineering community to select them. As such, impact of quality of code repositories on the performance of these systems needs to be studied. In this preliminary paper, we evaluate impact of different quality repositories on the performance of a candidate MP system. Towards that objective, we develop a framework, named GitRank, to rank open-source repositories on quality, maintainability, and popularity by leveraging existing research on this topic. We then apply GitRank to evaluate correlation between the quality measures used by the candidate MP system and the quality measures used by our framework. Our preliminary results reveal some correlation between the quality measures used in GitRank and ControlFlag's performance, suggesting that some of the measures used in GitRank are applicable to ControlFlag. But it also raises questions around right quality measures for code repositories used in MP systems. We believe that our findings also generate interesting insights towards code quality measures that affect performance of MP systems.

==> impl.tex <==
\section{Implementation}
\label{section:impl}

{\framework} is implemented in Python, with implementation of phase 1 taking
around 400 lines of code, while that of phase 2 taking around 300 lines of code.
Phase 1 uses different approaches to obtain values of measures for repositories.
In particular, we use GitHub REST APIs~\cite{githubrestapi} to obtain the
number of stargazers, subscribers, forks, commits, and open and closed issues of
a repository. We use Python APIs of \texttt{lizard} project~\cite{lizard} to
obtain function-level cyclomatic complexity. As our formula for maintainability
index requires values of Halstead volume~\cite{halstead}, which are not
calculated by \texttt{lizard}, we extend \texttt{lizard} project with a plugin
to calculate those values. We use \texttt{cpplint} project~\cite{cpplint} to
obtain the number of style errors and use \texttt{FlawFinder}
tool~\cite{flawfinder} to obtain the security errors in C/C++ programs.

%We use Python programming language to implement our framework. Specifically,
%implementation of phase 1 of the framework that obtains repository-specific
%information is approximately 400 lines of Python code, while the implementation of
%second phase that ranks repositories is approximately 300 lines of code.


